Stochastic Non-preemptive Co-flow Scheduling with Time-Indexed Relaxation

Co-flows model a modern scheduling setting that is commonly found in a variety of applications in distributed and cloud computing. A stochastic co-flow task contains a set of parallel flows with randomly distributed sizes. Further, many applications require non-preemptive scheduling of co-flow tasks. This paper gives an approximation algorithm for stochastic non-preemptive co-flow scheduling. The proposed approach uses a time-indexed linear relaxation, and uses its solution to come up with a feasible schedule. This algorithm is shown to achieve a competitive ratio of $(2\log{m}+1)(1+\sqrt{m}\Delta)(1+m{\Delta}){(3+\Delta)}/{2}$ for zero-release times, and $(2\log{m}+1)(1+\sqrt{m}\Delta)(1+m\Delta)(2+\Delta)$ for general release times, where $\Delta$ represents the upper bound of squared coefficient of variation of processing times, and $m$ is the number of servers.

==> abstract.tex <==
\begin{abstract}
Co-flow scheduling problem has become popular for designing communication pattern in datacenters. In \cite{}, Chowdhury and Stoica designed the co-flow networking model describing the communication patterns. In \cite{Chowdhury:2014:ECS:2740070.2626315}, Chowdhury et al. introduced heuristic models for co-flow. \cite{Qiu:2015:MTW:2755573.2755592} and \cite{DBLP:journals/corr/ImP17} provided polynomial-time deterministic approximation algorithms for the preemptive co-flow scheduling problem. However, it is very possible that a task arriving has unknown size. A stochastic model is more practical for real world. Moreover, although preemptive scheduling is more effective in thoery, our computer systems are unable to avoid introducing performance loss taking into consideration of extra signaling overhead, flow switching latency, packet drops, limitation on hardware, etc. during implementation. Therefore, stochastic non-preemptive scenario is more widely implemented in practice. In our paper, we study a linear programming relaxation problem of stochastic co-flow scheduling problem without preemption. We show an approximation algorithm to minimize the expected total weighted completion time of all co-flow tasks. In this paper, we get an $(m(3+\Delta)+\epsilon)\log{m}$ approximation rate for zero-release time and $(2m(2+\Delta)+\epsilon)\log{m}$ approximation rate when tasks have release time, where $\Delta$ represents the upper bound of squared coefficient of variation of processing times, $m$ is the number of servers, and $\epsilon$ is arbitrarily small.
\end{abstract}

==> algorithm.tex <==
\section{Algorithm}
For non-preemptive, scheduling, the essential part is to decide the start time of all constituent flows. Our scheduling algorithm is summarized in Algorithm 1, consisting 4 steps. In Step 1, we solve our relaxed LP problem and get the probability for each constituent flow starting at each time slot. In Step 2, we generate tentative start time for each flow based on distribution we computed. In Step 3, we group all the flows with same tentative start time as a single time indexed co-flow, and further group each grouped flows into several perfect matching with Greedy Low Jitter decomposition algorithm to get a non-preemptive scheduling on for each time indexed co-flow . In Step 4, we sequence all time indexed co-flow. Namely, complete every required co-flow tasks according the sequence of modified time indexed co-flow.
\begin{table}[htbp]\centering
\begin{tabular}{l}
\hline Algorithm 1: Stochastic LP-based Approximation:\\
\hline
\textbf{Data}:  $p_{ijkt}$, $\mathbb{E}[T_{ijk}]$, for $i,j\in\mathcal{M},k\in\mathcal{M}$;\\
\textbf{Result}: A stochastic non-preemptive algorithm in polynomial time.\\
$\bullet$ Step 1: Solve our linear program: \\
\qquad get $y_{ijkt}$ from the LP solution, for $i,j\in\mathcal{M},k\in\mathcal{M}$;\\
$\bullet$ Step 2: For each flow $(i,j),i,j\in \mathcal{M}$ of coflow $k\in\mathcal{K}$:\\
\qquad choose $t$ independently with probability $y_{ijkt}$;\\
\qquad choose $r\in\mathbb{Z}_{\geq0}$ independently with probability $p_{ijkr}/\mathbb{E}[T_{ijk}]$;\\
\qquad denote $s:=t+r$ as tentative start time of flow on link $(i,j)$ of $k$\\
\qquad as $t(k,i,j)=s$.\\

$\bullet$ Step 3: Schedule all flows having same tentative start time by GLJD\\
\qquad  algorithm (Greedy Low Jitter decompostion algorithm).\\

$\bullet$ Step 4: Sequence all flows on all links by increasing tentative start \\
\qquad time order.\\
\hline
\end{tabular}
\end{table}

Before we give the algorithm of Greedy Low Jitter decomposition, we first explain the connection between non-preemptive co-flow scheduling on a single co-flow and NIQPMD (non-negative integral quasi-permutation matrix decompostion) on a non-negative matrix.

\begin{definition} [NIQPMD]

Suppose we decompose $D$ as $D=D^1+D^2+\cdots+D^k$, and the decomposition is a NIQPMD, we have:

$\bullet$ $ D^{l},\forall l\in[k]$ is non-negative, and has at most one nonzero element on each row and each column;

$\bullet$ If $D_{ij}>0$, only one matrix $D^{l'}$ has $D^{l'}_{ij}=D_{ij}$.
\end{definition}
The equivalence between non-preemptive co-flow scheduling on a single co-flow and NIQPMD is explained as following:

Every co-flow contains flows on all links between servers. Suppose we have $m$ servers, we can denote any co-flow as a $m$ by $m$ matrix $D$ with $D_{ij}$ is the size of data needed to be transmitted from server $i$ to server $j$, namely size of the constituent flow on link $(i,j)$. Non-preemptive scheduling of a single co-flow requires us to distribute constituent flows into groups, such that flows in each group can be processed at the same time (satisfying matching constriants $(3)$-$(4)$ in relaxed LP). If we complete all constituent flows group by group, the completion time of the non-preemptive scheduling for the co-flow is the summation of maximum processing time in each group. Any non-preemptive scheduling of single co-flow can be represented as a method to decompose a non-negative matrix to several non-negative quasi-permutation matrices, with every non-zero entry being distributed to one resulting matrix. Note that any quasi-permutation matrix represents a satisfaction of matching constriants: any server is the source of at most one flow, and the sink of at most one flow; the property that the existance of a resulting matrix $D^{l'}$ satisfying $D^{l'}_{ij}=D_{ij}$ for any  $D_{ij}>0$ guarantees the non-preemptive nature.


\begin{table}[htbp]\centering
\begin{tabular}{l}
\hline Algorithm 2: Greedy Low Jitter decomposition:\\
\hline
\textbf{Data}: Co-flow size matrix $D$ with $D_{ij}=\mathbb{E}($size of flow on $(i,j))$;\\
\textbf{Result}: Groups of permutation matrices $X^k$ and their size $m_k$;\\
$\bullet$ Step 1: Sort entries of $D$ in non-increaing order to creat a list $L$.\\
\qquad If $L(m)=D_{ij}$, set $\rho(m)=i$ and $\kappa(m)=j$. Initiate $k=1$;\\
$\bullet$ Step 2: \\
\qquad While $L\neq \emptyset$\\
\qquad \qquad Set $m_k=0$ and $l=1$\\
\qquad \qquad Set $C[j]=0$ $\forall j\in[n]$\\
\qquad \qquad While (Not end of list $L$)\\
\qquad \qquad \qquad While ($C[\rho(l)]=0 and C[\kappa(l)]=0$)\\
\qquad \qquad \qquad \qquad $X_{\rho(l)\kappa(l)}=1$\\
\qquad \qquad \qquad \qquad $C[\rho(l)]=C[\kappa(l)]=1$\\
\qquad \qquad \qquad \qquad If $L(l)>m_k$: $m_k=L(l)$\\
\qquad \qquad \qquad \qquad Eliminate entry $l$ from list $L$.\\
\qquad \qquad \qquad $l\leftarrow l+1$\\
\qquad \qquad $k\leftarrow k+1$\\
\hline
\end{tabular}
\end{table}

GLJD provides us a method of NIQPMD and returns each group's matching pairs and the maximum expectation of processing time among the pairs. GLJD algorithm first sort the expected size of each flow in non-increasing order to create a list $L$. Two elements are not conflict if they have no interference on source or sink servers. We greedily pick the flows from the top to the bottom of the list to form a quasi-permutation matrix as long as those elements are not conflict to each other. Once we finished searching the list for non-conflicting flows, we delete the corresponding elements from list $L$ and start searching for the next quasi-permutation matrix until the list $L$ become empty.





==> apdx1.tex <==
\section{Test}

==> conclusion.tex <==
\section{Conclusions}

==> intro.tex <==
\section{Introduction}
With the common use of parallel computation, parallel flows computation frameworks such as MapReduce\cite{Dean:2008:MSD:1327452.1327492}, Hadoop\cite{shvachko2010hadoop}, Spark and Google Dataflow are growing at unprecedented speed. Those powerful frameworks allows users from different places uploading and downloading huge amount of data at the same time. As cited by Gustavo Ambrozio, Lead Software Engineer of Pocket Gems: 'In minutes you might have hundreds of thousands of players playing your game. Google Cloud Platform allows us to scale automatically. We don't even have to think about it.'

Problem of optimizing better efficiency in scheduling tasks in those frameworks are introduced at the same time. \cite{chowdhury2011managing} showed that more than $50\%$ of time are spent during data transmission in practice. For instance, shuffle phase in MapReduce application has a large amount of data being transmitted between different servers at the same time. Given the matching limitation nature among servers, it is possible that some sets of data need to wait until the related ports become available. 

From the definition from \cite{Chowdhury:2012:CNA:2390231.2390237}, if we regard each server as a node, a co-flow task can be interpreted as a bipartite graph, with each node having capacity constraints and each constituent flow contained having size and link parameters. Co-flow scheduling assigns each constituent flows from all co-flow tasks according to their sizes, related server locations, and system capacity to all time slots. \cite{Chowdhury:2014:ECS:2740070.2626315} already proposed an efficient heuristic implementation.

Under non-preemptive constraints, each flow occupies whole capacity of its source and sink servers, namely one unit per time slot, until the completion of the flow. Non-preemptive co-flow model provides flexibility and efficiency based on parallelism: constituent flows from several co-flows might be processed at same time. On the other hand, non-preemptive co-flow model presents challenges with respect to the non-deterministic size, capacity constriants. \cite{yu2016non} is the first paper considering non-preemptive co-flow problem, where non-preemptive represents the data path and bandwidth share of a flow remain unchanged once started, and the bandwith of links between servers are given. However, our model assume the constraints are on input and output ports of each server instead of links, following the definition from \cite{Chowdhury:2012:CNA:2390231.2390237}. In our model,  each node (server / port) has at most one unit of work being processed at any time for both input and output.  Upon arrival of each co-flow task, we know nothing about the size of each constituent flow except of its distribution. We try to minimize the expected weighted time based on distribution.

Our paper provides the first algorithm for stochastic co-flow scheduling problem without preemption. 

The rest of this paper is organized as following. Section II introduces related work of co-flow scheduling and input-queued switches in the literature. Section III presents the system model and a relaxed linear programming problem for the model.  Section IV presents the proposed
algorithm, including generating a tentative start time and further sequencing all of flows to get a feasible scheduling based on the LP solutions. Section V gives the approximation rate between our feasible solution and optimal solution. Secion VI concludes the paper.


==> model.tex <==
\section{System Model}
A co-flow task is a set of parallel flows that need to be completed in a bipartite network. The completion of a co-flow task needs the completion of all constituent flows. Co-flow task has all start and end ports assigned to each constituent flow, while having less information about the size of each flow. Each port has capacity constraint: both its start port and end port can only have one flow being processed at any time point. We get to know the size of each flow upon the start 

We derive an LP relaxation of the stochastic non-preemptive co-flow scheduling problem as following:
$y_{ijkt}$: probability that the schedule starts flow on link $(i,j)$ from coflow task $k$ on at time $t\in\mathbb{Z}_{\geq0}$;

$T_{ijk}$: random variable representing the processing time of flow on link $(i,j)$ from coflow task $k$;

$p_{ijks-t}$: given flow on link $(i,j)$ from coflow task $k$ started at time $t$, the probability that k is still being processed during time slot $[s,s+1]$.

\begin{align}
& \min &&\sum_{k\in\mathcal{K}} w_kC_k^{LP} \nonumber\\
& \rm{s.t.} && \sum_{t\in\mathbb{Z}_{\geq0}}y_{ijkt}=1 \nonumber\\
&  &&\qquad\qquad \forall i,j\in\mathcal{M},\quad\forall k\in\mathcal{K};\\
& &&\sum_{j\in\mathcal{M}}\sum_{k\in\mathcal{K}}\sum_{t=0}^s y_{ijkt}p_{ijks-t}\leq 1\nonumber\\
&  &&\qquad\qquad\forall i\in\mathcal{M},\quad s\in\mathbb{Z}_{\geq0};\\
& &&\sum_{i\in\mathcal{M}}\sum_{k\in\mathcal{K}}\sum_{t=0}^s y_{ijkt}p_{ijks-t}\leq 1\nonumber\\
&  &&\qquad\qquad\forall j\in\mathcal{M},\quad s\in\mathbb{Z}_{\geq0};\\
& &&C_k^{LP}\geq \sum_{t\in\mathbb{Z}_{\geq0}} y_{ijkt}(t+\mathbb{E}[T_{ijk}])\nonumber \\
& &&\qquad\qquad \forall i,j\in\mathcal{M},\quad\forall k\in\mathcal{K};\\
& && y_{ijkt}\geq 0\nonumber\\
& &&\qquad\qquad \forall i,j\in\mathcal{M},\quad\forall k\in\mathcal{K},\quad t\in\mathbb{Z}_{\geq0}.
\end{align}
Constraint $(1)$ says that every co-flow task $k$'s constituent flow on link $(i,j)$ will be assigned some time; constraint $(2)$ and $(3)$ are matching constraints: at any time slot, for any server, at most one unit of data can be received and at most one unit of data can be sent; constraint $(4)$ says the completion time of a co-flow task is the maximum among all of its constituent coflow completion time; constraint $(5)$ says probability that the schedule starts flow on any link $(i,j)$ from any coflow task $k$ on at any time $t\in\mathbb{Z}_{\geq0}$ is non-negative.

==> proofs.tex <==
\section{Approximation Guarantees}
Now we show our approximation bound for our scheduling algorithm.
\begin{theorem}
The completion time of every coflow task $k$ under our scheduling algorithm is at most  $C_k^{LP}(3+\Delta)\log{m}$ where $\Delta$ is the upper bound of $\Delta_{ij}$ for all $i,j\in \mathcal{M}$, and $m$ is the number of servers.
\end{theorem}

Before the proof, we give a definition of efficient size for co-flow.

\begin{definition}[Efficient Size]
Any co-flow can be denoted as a matrix $D\in\mathbb{R}^{m\times m}$ with its entry $D_{ij}$ representing the size of its constituent flow from server $i$ to server $j$. The efficient size of a co-flow is the maximum of its maximum columns sum and its maximum rows sum in its representative matrix. Namely, the efficient size of $D$ is:
\begin{equation*}
\max\Big{\{}\max_i\sum_j D_{ij},\max_j\sum_i D_{ij}\Big{\}}.
\end{equation*}
\end{definition}

To prove theorem, we use four lemmas. The first lemma is to prove that for all flows having same tentative time, the co-flow formed by them has expected efficient size less or equal to $1$. If we assume the expected time to process a stochastic co-flow with expected efficient size less or equal to $1$ has upper bound $T$, then the summation of expected time scheduled before any flow with tentative start time $s$ has upper bound $(s+1/2)T$.
\begin{lemma}
Assume the expected time to process a stochastic co-flow with expected efficient size less or equal to $1$ has upper bound $T$. For any $i,j\in\mathbb{M}$, $k\in\mathcal{K}$, and $s\in\mathbb{Z}_{\geq0}$, if $t(k,i,j)=s$, then the summation of expected time scheduled before coflow $k$ is less or equal to $(s+1/2)T$.
\end{lemma}
\begin{proof}
From the scheduling policy, we have
\begin{equation*}
Pr[t(k,i,j)=s]=\sum_{t=0}^s y_{ijkt}\frac{p_{ijks-t}}{\mathbb{E}[T_{ijk}]}.
\end{equation*}
From the above equation and constraint $(2)-(3)$, we have the following:
\begin{align*}
&\max_i\sum_j\sum_{k'\neq k}\mathbb{E}[T_{ijk'}]Pr[t(k',i,j)=s']\\
=&\max_i\sum_j\sum_{k'\neq k}\sum_{t'=0}^{s'}y_{ijk't'}p_{ijk's'-t'}\leq 1;
\end{align*}
and
\begin{align*}
&\max_j\sum_i\sum_{k'\neq k}\mathbb{E}[T_{ijk'}]Pr[t(k',i,j)=s']\\
=&\max_j\sum_i\sum_{k'\neq k}\sum_{t'=0}^{s'}y_{ijk't'}p_{ijk's'-t'}\leq 1.
\end{align*}
If we consider the set of flows with same tentative start time as a co-flow, the co-flow has expected efficient size less or equal to $1$. From the assumption, the expected processing time is upper bounded by $T$.
Therefore, the summation of expected time scheduled before coflow $k$ is bounded by $(s+1/2)T$.
\end{proof}


From the definition of $p_{ijks-t}$ and $T_{ijk}$, we have the relation:
\begin{equation*}
p_{ijkr}:=Pr[T_{ijk}\geq r+1]\qquad \forall i,j\in{\mathcal{M}},~\forall k\in\mathcal{K},~\rm{and}~\forall r\in\mathbb{Z}_{\geq 0}.
\end{equation*}
The following lemma helps to prove theroem.
\begin{lemma}
For every $i,j\in\mathcal{M}$, $k\in\mathcal{K}$ and $r\in\mathbb{Z}_{\geq 0}$, we have
\begin{equation*}
\sum_{r\in\mathbb{Z}_{\geq 0}}(r+\frac{1}{2})\frac{q_{ijkr}}{\mathbb{E}[T_{ijk}]}=\frac{1+\mathbb{CV}[T_{ijk}]^2}{2}\mathbb{E}[T_{ijk}],
\end{equation*}
where $\mathbb{CV}[P_{ijk}]^2$ is $P_{ijk}$'s squared coefficient of variation.
\end{lemma}


The following two lemmas helps to prove the last lemma which gives a proper upper bound for $T$ given in lemma 1.

The following lemma is from \cite{keslassy2003guaranteed} theorem 6, giving us a guarantee for deterministic non-preemptive scheduling with efficient size less or equal to $1$.
\begin{lemma}
Let the server number $m\geq 2$, the maximum total weights decomposed from a matrix $D$ with $\max\Big{\{}\max_i\sum_j D_{ij},\max_j\sum_i D_{ij}\Big{\}}$ is less or equal to $2\log{m}+1$.
\end{lemma}


\begin{lemma}[Devroye\cite{}]
If $X_1,X_2,\cdots,X_m$ are $m$ random variables with finite means and finite variances, then 
\begin{equation*}
\mathbb{E}[\max_{i} X_i]\leq \max_i \mathbb{E}[Y_i]+\sqrt{m}\max_i\sqrt{Var(X_i)},
\end{equation*}
\end{lemma}

Now we give a proper upper bound $T$ in Lemma 1.
\begin{lemma}
Suppose we have $m$ servers, then the expected time to process a stochastic co-flow with expected efficient size less or equal to $1$ has upper bound $(2\log{m}+1)(1+\sqrt{m\Delta})$, where  $\Delta$ is the upper bound of squared coefficient of variation of all processing time.
\end{lemma}
\begin{proof}
Given the set of stochastic flows forming a stochasic co-flow, we use their expected size for GLJD algorithm, and return groups of flows with each group being processed simultaneously. GLJD returns the maximum expected size of flows in each group. However, the expected processing time for each group is the expectation of the maximum of the random sizes. Lemma 4 bridge the gap between $\mathbb{E}[max_i X_i]$ and $\max_i\mathbb{E}[X_i]$ with $(1+\sqrt{m\Delta})$. Therefore the $T$ mentioned in Lemma 1 can be the multiplication of the gap between GLJD returned processing time and $(1+\sqrt{m\Delta})$.
\end{proof}


\begin{proof}[proof for Theorem 1]
Let

 $\mathbb{E}[C_{(k,i,j)}]=\sum_{t\in\mathbb{Z}_{\geq0}} y_{ijkt}(t+\mathbb{E}[T_{ijk}])$.
\begin{align*}
\mathbb{E}[C_{(k,i,j)}]&=\sum_{i,j\in\mathcal{M}}\sum_{s\in\mathbb{Z}_{\geq 0}}\mathbb{E}[C_{(k,i,j)}|t(k,i,j)=s]Pr[t(k,i,j)=s]\\
&\leq\sum_{i,j\in\mathcal{M}}\sum_{s\in\mathbb{Z}_{\geq 0}}\Big{(}T(s+\frac{1}{2})+\mathbb{E}[T_{ijk}]\Big{)}\sum_{t=0}^s y_{ijkt}\frac{p_{ijks-t}}{\mathbb{E}[T_{ijk}]}\\
&\leq T\sum_{i,j\in\mathcal{M}}\sum_{t\in\mathbb{Z}_{\geq 0}}y_{ijkt}\Big{(}t+\mathbb{E}[T_{ijk}]+\sum_{r\in\mathbb{Z}_{\geq 0}}(r+\frac{1}{2})\frac{p_{ijkr}}{\mathbb{E}[T_{ijk}]}\Big{)}\\
&=T\sum_{i,j\in\mathcal{M}}\sum_{t\in\mathbb{Z}_{\geq 0}}y_{ijkt}\Big{(}t+\Big{(}\frac{3}{2}+\frac{\mathbb{CV}[T_{ijk}]^2}{2}\Big{)}\mathbb{E}[T_{ijk}]\Big{)}\\
&\leq(2\log{m}+1)(1+\sqrt{m\Delta})\frac{3+\Delta_{ij}}{2}C_{(k,i,j)}^{LP}.
\end{align*}
Since $\mathbb{E}[C_k]=\max_{i,j\in\mathcal{M}}\mathbb{E}[C_{(k,i,j)}]\leq \max_{i,j\in\mathcal{M}}C_{(k,i,j)}^{LP}(2\log{m}+1)(1+\sqrt{m\Delta})\Big{(}\frac{3+\Delta_{ij}}{2}C_{(k,i,j)}^{LP}\Big{)}\leq C_k^{LP}(2\log{m}+1)(1+\sqrt{m\Delta})\Big{(}\frac{3+\Delta_{ij}}{2}C_{(k,i,j)}^{LP}\Big{)}$, where $\Delta$ is the upper bound of $\Delta_{ij}$ for all $i,j\in \mathcal{M}$, $m$ is the number of servers.
\end{proof}



==> related.tex <==
\section{Related Work}
\subsection{Co-flow Scheduling}
The concept of co-flow is first proposed in 2012 by Chowdhury\cite{Chowdhury:2012:CNA:2390231.2390237}. \cite{Chowdhury:2014:ECS:2740070.2626315} proposed an efficient heuristic implementation. 

For theoretical bound of deterministic preemptive co-flow scheduling, \cite{Qiu:2015:MTW:2755573.2755592}, \cite{shafiee2017scheduling} and \cite{DBLP:journals/corr/ImP17} provided polynomial-time deterministic approximation algorithms for the preemptive co-flow scheduling problem. In \cite{Qiu:2015:MTW:2755573.2755592}, Qiu et al. use a relaxed linear programming result to get reference on co-flow seqences to be completed, and use Birkhoff-von-Neumann decompositon theorem to assign flows preemptively. 

For theoretical bound of deterministic preemptive co-flow scheduling, \cite{yu2016non} provided a version of deterministic non-preemptive scheduling with known link bandwidth and stable bandwidth assigned to each started flow.
\subsection{Input-queued switch}
To decrease the frequency of matching computation for crossbar configuration in high-speed core routers, frame-based scheduling is being studied. One of the essential steps of frame-based scheduling is the computation of a list of input/output pair. The pairing step is similar to co-flow scheduling in the sense of grouping constituent flows to be processed at the same time slot. The listing step is similar to co-flow scheduling in the sense of sequencing the groups flows at each time slot. \cite{keslassy2003guaranteed} introduced Greedy Low Jitter Decomposition Algorithm to solve list pairing scheduling problem. The GLJD algorithm can be seen as a correspondence to Birkhoff-von-Neumann decomposition theorem where GLJD is for non-preemptive scheduling while BV is for preemptive scheduling.
\subsection{Stochastic scheduling on parallel machines}
For co-flow scheduling, it is impossible to schedule incoming co-flow tasks as off-line circumstances in practice. Introducing stochastic variant of co-flow scheduling is natural. In 1966, \cite{rothkopf1966scheduling} proved that WSEPT rule (weighted shortest expected processing time first) is optimal for minimizing weighted completion time on single server.Based onWSEPT rule, \cite{skutella2016unrelated} studies the stochastic variant of unrelated parallel machine scheduling for the first time.  The time-indexed linear programming relaxation for stochastic machine scheduling inspired us to further study the stochastic case in non-preemptive co-flow scheduling.

==> tmp_docsiamart_abstract.tex <==
\begin{abstract}
Co-flow scheduling problem has become popular for designing communication pattern in datacenters. In \cite{}, Chowdhury and Stoica designed the co-flow networking model describing the communication patterns. In \cite{Chowdhury:2014:ECS:2740070.2626315}, Chowdhury et al. introduced heuristic models for co-flow. \cite{Qiu:2015:MTW:2755573.2755592} and \cite{DBLP:journals/corr/ImP17} provided polynomial-time deterministic approximation algorithms for the preemptive co-flow scheduling problem. However, it is very possible that a task arriving has unknown size. A stochastic model is more practical for real world. Moreover, although preemptive scheduling is more effective in thoery, our computer systems are unable to avoid introducing performance loss taking into consideration of extra signaling overhead, flow switching latency, packet drops, limitation on hardware, etc. during implementation. Therefore, stochastic non-preemptive scenario is more widely implemented in practice. In our paper, we study a linear programming relaxation problem of stochastic co-flow scheduling problem without preemption. We show an approximation algorithm to minimize the expected total weighted completion time of all co-flow tasks. In this paper, we get an $(2\log{m}+1)(1+\sqrt{m\Delta}){(3+\Delta_{ij})}/{2}+\epsilon$ approximation rate for zero-release time and  approximation rate $(2\log{m}+1)(1+\sqrt{m\Delta}){(2+\Delta_{ij})}+\epsilon$when tasks have release time, where $\Delta$ represents the upper bound of squared coefficient of variation of processing times, $m$ is the number of servers, and $\epsilon$ is arbitrarily small.
\end{abstract}

\begin{keywords}
TBD
\end{keywords}

\begin{AMS}
TBD
\end{AMS}


==> tmp_docsiamart_alg.tex <==
\begin{algorithm}
\caption{Build tree}
\label{alg:buildtree}
\begin{algorithmic}[1]
\STATE{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\WHILE{$\#P > 1$}
\STATE\label{line3}{Choose $C^\prime\in\mathcal{C}_p(P)$ with $C^\prime := \operatorname{argmin}_{C\in\mathcal{C}_p(P)} \varrho(C)$}
\STATE{Find an optimal partition tree $T_{C^\prime}$ }
\STATE{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\STATE{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus} \mathcal{L}(T_{C^\prime})\}$}
\ENDWHILE
\RETURN $T$
\end{algorithmic}
\end{algorithm}


==> tmp_docsiamart_fig.tex <==
\begin{figure}[tbhp]
  \centering
  \subfloat[$\epsilon_{\max}=5$]{\label{fig:a}\includegraphics{lexample_fig1}}
  \subfloat[$\epsilon_{\max}=0.5$]{\label{fig:b}\includegraphics{lexample_fig2}}
  \caption{Example figure using external image files.}
  \label{fig:testfig}
\end{figure}


==> tmp_docsiamart_header.tex <==

% Custom SIAM macro to insert headers
\title{Stochastic Co-flow Scheduling with Time-Indexed Relaxation}
\author{Ruijiu Mao and Vaneet Aggarwal\thanks{R. Mao and V. Aggarwal are with Purdue University, West Lafayette IN 47907 (email: mao95@purdue.edu, vaneet@purdue.edu). }}


==> tmp_docsiamart_simpletable.tex <==
\begin{table}[tbhp]
  \caption{Example table}
  \label{tab:simpletable}
  \centering
  \begin{tabular}{|c|c|c|} \hline
   Species & \bf Mean & \bf Std.~Dev. \\ \hline
    1 & 3.4 & 1.2 \\
    2 & 5.4 & 0.6 \\ \hline
  \end{tabular}
\end{table}


==> tmp_docsiamart_table.tex <==
\newcolumntype{R}{>{$}r<{$}}  %
\newcolumntype{V}[1]{>{[\;}*{#1}{R@{\;\;}}R<{\;]}} %
\begin{table}[tbhp]
 \captionsetup{position=top} %<- Needed for using subtables created with the subfig package
  \caption{Example table adapted from Kolda and Mayo \rm{\cite{KoMa14}}.}
  \label{tab:KoMa14}
  \centering
  \subfloat[$\beta=1$]{
    \begin{tabular}{|r|R|V{3}|c|r@{\,$\pm$\,}l|} \hline
occ. & \multicolumn{1}{c|}{$\lambda$} & \multicolumn{4}{c|}{$\mathbf{x}$} &
fevals &  \multicolumn{2}{c|}{time (sec.)}\\ \hline
 718 & 11.3476 &  0.5544 &  0.3155 &  1.2018 &  0.0977 &   45 & 0.17 & 0.06 \\ \hline
 134 &  3.7394 &  0.2642 & -1.1056 &  0.2657 & -0.3160 &   31 & 0.12 & 0.05 \\ \hline
   4 & \multicolumn{6}{c|}{\emph{--- Failed to converge ---}} & 0.21 & 0.10 \\ \hline
 \end{tabular}}

  \subfloat[$\beta=-1$]{
    \begin{tabular}{|r|R|V{3}|c|r@{\,$\pm$\,}l|} \hline
occ. & \multicolumn{1}{c|}{$\lambda$} & \multicolumn{4}{c|}{$\mathbf{x}$} &
fevals &  \multicolumn{2}{c|}{time (sec.)}\\ \hline
  72 & -1.1507 &  0.2291 &  0.6444 &  0.3540 & -0.8990 &   34 & 0.14 & 0.06 \\ \hline
 624 & -6.3985 &  0.1003 &  0.1840 &  0.5305 &  1.2438 &   48 & 0.19 & 0.08 \\ \hline
   2 & \multicolumn{6}{c|}{\emph{--- Failed to converge ---}} & 0.23 & 0.02 \\ \hline
 \end{tabular}}
\end{table}


==> tmp_docsiamart_tikz.tex <==
\begin{figure}[tbhp]
  \centering
  \begin{tikzpicture}
    \begin{loglogaxis}[height=2.75in, grid=major,
      xlabel={Degrees of Freedom}, ylabel={$L_2$ Error},
      legend entries={$d=2$,$d=3$}]
      \addplot table [x=d2_dof,y=d2_l2_err] {data.dat};
      \addplot table [x=d3_dof,y=d3_l2_err] {data.dat};
    \end{loglogaxis}
  \end{tikzpicture}
  \caption{Example \texttt{PGFPLOTS} figure.}
  \label{fig:pgfplots}
\end{figure}

